On quantile residuals in beta regression

Beta regression is often used to model the relationship between a dependent variable that assumes values on the open interval (0,1) and a set of predictor variables. An important challenge in beta regression is to find residuals whose distribution is well approximated by the standard normal distribution. Two previous works compared residuals in beta regression, but the authors did not include the quantile residual. Using Monte Carlo simulation techniques, this paper studies the behavior of certain residuals in beta regression in several scenarios. Overall, the results suggest that the distribution of the quantile residual is better approximated by the standard normal distribution than that of the other residuals in most scenarios. Three applications illustrate the effectiveness of the quantile residual.

==> bibquant_v02.tex <==
@Article{abd+uma07,
 author  = {A. G. Abdul-Muhmin and Y. A. Umar},
 title   = {Credit card ownership and usage behaviour in Saudi Arabia: the impact of demographics and attitudes},
 journal = {Journal of Financial Services Marketing},
 volume  = {12},
 number  = {},
 pages   = {219-234},
 year    = {2007},
}

@Article{ait55,
 author  = {John Aitchison},
 title   = {On the distribution of a positive random variable having a discrete probability mass at the origin},
 journal = {Journal of the American Statistical Association},
 volume  = {50},
 number  = {},
 pages   = {901-908},
 year    = {1955},
}

@Article{aka74,
 author  = {Hirotugu Akaike},
 title   = {A new look at the statistical model identification},
 journal = {IEEE Transactions on Automatic Control},
 volume  = {19},
 number  = {6},
 pages   = {716-723},
 year    = {1974},
}

@Article{ame73,
 author  = {Takeshi Amemiya},
 title   = {Regression analysis when the dependent variable is truncated normal},
 journal = {Econometrica},
 volume  = {41},
 number  = {6},
 pages   = {997-1016},
 year    = {1973},
}

@Article{ame+bos74,
 author  = {Takeshi Amemiya and Michael Boskin},
 title   = {Regression analysis when the dependent variable is truncated lognormal with an application to the determinants of the duration of welfare dependency},
 journal = {International Economic Review},
 volume  = {15},
 number  = {2},
 pages   = {485-496},
 year    = {1974},
}



@mastersthesis{and07,
Author = {Augusto G. C. Andrade},
Title = {Efeitos da especificação incorreta da função de ligação no modelo de regressão beta},
School = {Instituto de Matemática e Estatística - Universidade de São Paulo},
Year = {2007},
Type = {Dissertação de mestrado em estatística},
}

@mastersthesis{anh10,
Author = {Tatiana Anholeto},
Title = {Resíduos de Pearson melhorados em modelos de regressão beta},
School = {Instituto de Matemática e Estatística - Universidade de São Paulo},
Year = {2010},
Type = {Dissertação de mestrado em estatística},
}

@Article{anh+san+bot14,
 author  = {T. Anholeto and M. C. Sandoval and D. A. Botter},
 title   = {Adjusted Pearson residuals in beta regression models},
 journal = {Journal of Statistical Computation and Simulation},
 volume  = {84},
 number  = {5},
 pages   = {999-1014},
 year    = {2014},
}

@Book{atk85,
 author  = {A. C. Atkinson},
 title   = {Plots, transformations and regression},
 edition = {},
 publisher={Clarendon Press},
 address = {Oxford},
 year    = {1985},
}

@online{ATP94,
  author = {{ATP Tour Inc}},
  title = {ATP Scores and Stats},
  year = {1994},
  url = {http://www.atpworldtour.com/en/stats},
  note = {Accessed: 2015-11-07}
}

@Article{bar+jor91,
 author  = {O. E. Barndorff-Nielsen and B. Jorgensen},
 title   = {Some parametric models on the simplex},
 journal = {Journal of Multivariate Analysis},
 volume  = {39},
 number  = {},
 pages   = {106-116},
 year    = {1991},
}

@Article{bay+cri13,
 author  = {F. M. Bayer and F. Cribari-Neto},
 title   = {Bartlett corrections in beta regression models},
 journal = {Journal of Statistical Planning and Inference},
 volume  = {143},
 number  = {},
 pages   = {531-547},
 year    = {2013},
}

@article{bayes2012new,
  title={A new robust regression model for proportions},
  author={Bayes, Cristian L and Baz{\'a}n, Jorge L and Garc{\'\i}a, Catalina and others},
  journal={Bayesian Analysis},
  volume={7},
  number={4},
  pages={841--866},
  year={2012},
  publisher={International Society for Bayesian Analysis}
}

@Article{bra+joh+thu07,
 author  = {Adam J. Branscum and W. O. Johnson and M. C. Thurmond},
 title   = {Bayesian beta regression: applications to household expenditure data and genetic distance between foot-and-mouth disease viruses},
 journal = {Australian and New Zealand Journal of Statistics},
 volume  = {49},
 number  = {3},
 pages   = {287-301},
 year    = {2007},
}

@Article{car+fer+val14,
 author  = {J. M. F. Carrasco and S. L. P. Ferrari and R. B. Arellano-Valle},
 title   = {Errors-in-variables beta regression models},
 journal = {Journal of Applied Statistics},
 volume  = {41},
 number  = {7},
 pages   = {1530-1547},
 year    = {2014},
}

@Article{coo86,
 author  = {R. D. Cook},
 title   = {Assessment of local influence (with discussion)},
 journal = {Journal of the Royal Statistical Society Series B},
 volume  = {48},
 number  = {},
 pages   = {133-169},
 year    = {1986},
}



@Article{coo+kie+mcc08,
 author  = {Douglas O. Cook and Robert Kieschnick and B. D. McCullough},
 title   = {Regression analysis of proportions in finance with self selection},
 journal = {Journal of Empirical Finance},
 volume  = {15},
 number  = {5},
 pages   = {860-867},
 year    = {2008},
}

@Article{cox96,
 author  = {Christopher Cox},
 title   = {Nonlinear quasi-likelihood models: applications to continuous proportions},
 journal = {Computational Statistics and Data Analysis},
 volume  = {21},
 number  = {},
 pages   = {449-461},
 year    = {1996},
}

@Article{cox+rei87,
 author  = {D. R. Cox and N. Reid},
 title   = {Parameter Orthogonality and Approximate Conditional Inference},
 journal = {Journal of the Royal Statistical Society Series B},
 volume  = {49},
 number  = {1},
 pages   = {1-39},
 year    = {1987},
}

@Article{cri+que14,
 author  = {F. Cribari-Neto and M. P. F. Queiroz},
 title   = {On testing inference in beta regressions},
 journal = {Journal of Statistical Computation and Simulation},
 volume  = {84},
 number  = {1},
 pages   = {186-203},
 year    = {2014},
}

@Article{cri+zei10,
 author  = {F. Cribari-Neto and A. Zeileis},
 title   = {Beta regression in R},
 journal = {Journal of Statistical Software},
 volume  = {34},
 number  = {2},
 pages   = {1-24},
 year    = {2010},
}


@Book{dor07,
 author  = {J. A. Doornik},
 title   = {An Object-Oriented Matrix Language: Ox 5},
 edition = {},
 publisher={Timberlake Consultants Press},
 address = {London},
 year    = {2007},
}

@Article{dow+nor03,
 author  = {W. H. Dow and E. C. Norton},
 title   = {Choosing between and interpreting the Heckit and
 two-part models for corner solutions},
 journal = {Health Services \& Outcomes Research Methodology},
 volume  = {4},
 number  = {},
 pages   = {5-18},
 year    = {2003},
}

@Article{dun+smy96,
 author  = {P. K. Dunn and G. K. Smyth},
 title   = {Randomized quantile residuals},
 journal = {Journal of Computational and Graphical Statistics},
 volume  = {5},
 number  = {3},
 pages   = {236-244},
 year    = {1996},
}

@Article{esp+fer+cri08a,
 author  = {P. L. Espinheira and S. L. P. Ferrari and F. Cribari-Neto},
 title   = {On beta regression residuals},
 journal = {Journal of Applied Statistics},
 volume  = {35},
 number  = {4},
 pages   = {407-419},
 year    = {2008},
}

@Article{esp+fer+cri08b,
 author  = {P. L. Espinheira and S. L. P. Ferrari and F. Cribari-Neto},
 title   = {Influence diagnostics in beta regression regression},
 journal = {Computational Statistics and Data Analysis},
 volume  = {52},
 number  = {9},
 pages   = {4417-4431},
 year    = {2008},
}

@Article{esp+fer+cri14,
 author  = {P. L. Espinheira and S. L. P. Ferrari and F. Cribari-Neto},
 title   = {Bootstrap prediction intervals in beta regressions},
 journal = {Computational Statistics},
 volume  = {29},
 number  = {},
 pages   = {1263-1277},
 year    = {2014},
}

@Article{fag+hos+bof08,
 author  = {Morten W. Fagerland and David W. Hosmer and Anna M. Bofin},
 title   = {Multinomial goodness-of-fit tests for logistic regression models},
 journal = {Statistics in Medicine},
 volume  = {27},
 number  = {},
 pages   = {4238-4253},
 year    = {2008},
}

@Article{fer+cri04,
 author  = {S. L. P. Ferrari and F. Cribari-Neto},
 title   = {Beta regression for modelling rates and proportions},
 journal = {Journal of Applied Statistics},
 volume  = {31},
 number  = {7},
 pages   = {799-815},
 year    = {2004},
}

@Article{feu79,
 author  = {Andrey Feuerverger},
 title   = {On some methods of analysis for weather experiments},
 journal = {Biometrika},
 volume  = {66},
 number  = {3},
 pages   = {655-658},
 year    = {1979},
}

@Article{fig+are+fer13,
 author  = {J. I. Figueroa-Zúñiga and R. B. Arellano-Valle and S. L. P. Ferrari},
 title   = {Mixed beta regression: A Bayesian perspective},
 journal = {Computational Statistics and Data Analysis},
 volume  = {61},
 number  = {},
 pages   = {137-147},
 year    = {2013},
}


@Techreport{gre94,
 author  = {W. H. Greene},
 title   = {Accounting for excess zeros and sample selection in Poisson and negative binomial regression models},
institution = {Department of Economics, New York University},
year    = {1994},
Type = {Working papers EC-94-10},
}

@Book{gre08,
 author  = {W. H. Greene},
 title   = {Econometric analysis},
 edition = {7},
 publisher={Prentice Hall},
 address = {New York},
 year    = {2008},
}

@Book{gup+nad04,
 author  = {Arjun K. Gupta and Saralees Nadarajah},
 title   = {Handbook of beta distribution and its applications},
 edition = {},
 publisher={Marcel Dekker},
 address = {New York},
 year    = {2004},
}

@Article{hall00,
 author  = {D. B. Hall},
 title   = {Zero-inflated Poisson and binomial regression with random effects: a case study},
 journal = {Biometrics},
 volume  = {56},
 number  = {},
 pages   = {1030-1039},
 year    = {2000},
}

@Article{ham+kha01,
 author  = {R. Hamilton and M. Khan},
 title   = {Revolving credit card holders: who are they and how can be identified},
 journal = {The Services Industries Journal},
 volume  = {21},
 number  = {3},
 pages   = {37-48},
 year    = {2001},
}

@Book{har+hil03,
 author  = {James W. Hardin and Joseph M. Hilbe},
 title   = {Generalized estimating equations},
 edition = {},
 publisher={Chapman and Hall},
 address = {Boca Raton},
 year    = {2003},
}

@inproceedings{hel+sta+rig06,
 author  = {G. Heller and M. Stasinopoulos and B. Rigby},
 title   = {The zero-adjusted Inverse Gaussian distribution as a model for insurance claims},
 booktitle = {21th International Workshop on Statistical Modelling},
 address = {Galway:Ireland},
 note = {226-233},
 year = {2006},
}

@Article{her+wal94,
 author  = {Benjamin E. Hermalin and Nancy E. Wallace},
 title   = {The determinants of efficiency and solvency in saving and loans},
 journal = {The RAND Journal of Economics},
 volume  = {25},
 number  = {3},
 pages   = {361-381},
 year    = {1994},
}


@Article{hof07,
 author  = {A. Hoff},
 title   = {Second stage DEA: Comparison of approaches for modelling the DEA escore},
 journal = {European Journal of Operational Research},
 volume  = {181},
 number  = {},
 pages   = {425-435},
 year    = {2007},
}

@Book{hos+lem00,
 author  = {David W. Hosmer and Stanley Lemeshow},
 title   = {Applied logistic regression},
 edition = {Second},
 publisher={John Wiley and Sons},
 address = {New York},
 year    = {2000},
}

@Book{joh+kot+bal95,
 author  = {Norman L. Johnson and Samuel Kotz and N. Balakrishnan},
 title   = {Continuous univariate distributions},
 edition = {Second},
 publisher={John Wiley and Sons},
 address = {New York},
 year    = {1995},
}

@Book{joh+wic07,
 author  = {R. A. Johnson and D. W. Wichern},
 title   = {Applied Multivariate Statistical Analysis},
 edition = {6},
 publisher={Prentice Hall},
 address = {Upper Saddle River},
 year    = {2007},
}

@Article{jon08,
 author  = {R. Jonsson},
 title   = {When does Heckman´s two step-procedure for censored data work and when does it not?},
 journal = {Statistical Papers},
 volume  = {, in press},
 number  = {},
 pages   = {},
 year    = {2010},
}

@Article{jor97a,
 author  = {B. Jorgensen},
 title   = {Proper dispersion models (with discussion)},
 journal = {Brazilian Journal of Probability and Statistics},
 volume  = {11},
 number  = {2},
 pages   = {89-140},
 year    = {1997},
}

@Book{jor97b,
 author  = {B. Jorgensen},
 title   = {The theory of dispersion models},
 edition = {},
 publisher={Chapman and Hall},
 address = {London},
 year    = {1997},
}

@Article{kum80,
 author  = {P. Kumaraswamy},
 title   = {A generalized probability density function for double-bounded random processes},
 journal = {Journal of Hydrology},
 volume  = {46},
 number  = {},
 pages   = {79-88},
 year    = {1980},
}

@Article{kie+mcc03,
 author  = {R. Kieschnick and B. D. McCullough},
 title   = {Regression analysis of variates observed on (0,1): percentages, proportions and fractions},
 journal = {Statistical Modelling},
 volume  = {3},
 number  = {},
 pages   = {193-213},
 year    = {2003},
}

@Article{kim+dev01,
 author  = {H. Kim and S. A. DeVaney},
 title   = {The determinants of outstanding balances among credit card revolvers},
 journal = {Financial Counseling and Planning},
 volume  = {12},
 number  = {1},
 pages   = {67-77},
 year    = {2001},
}

@Article{lam92,
 author  = {D. Lambert},
 title   = {Zero-inflated Poisson regression, with an application to defects in manufacturing},
 journal = {Technometrics},
 volume  = {34},
 number  = {},
 pages   = {1-14},
 year    = {1992},
}

@article{latif2015d,
  title={D-optimal designs for beta regression models with single predictor},
  author={Latif, Shahid and Zafar Yab, Mohammad},
  journal={Journal of Statistical Computation and Simulation},
  volume={85},
  number={9},
  pages={1709--1724},
  year={2015},
  publisher={Taylor \& Francis}
}

@Book{leh+cas98,
 author  = {E. L Lehmann and George Casella},
 title   = {Theory of point estimation},
 edition = {2},
 publisher={Springer-Verlag},
 address = {New York},
 year    = {1998},
}

@article{lemonte2015new,
  title={New class of Johnson SB distributions and its associated regression model for rates and proportions},
  author={Lemonte, Artur J and Baz{\'a}n, Jorge L},
  journal={Biometrical Journal},
  volume  = {58},
  number  = {4},
  pages   = {727-746},    
  year={2016},
  publisher={Wiley Online Library}
}

@Article{les+riz+tso07,
 author  = {Emmanuel Lesaffre and Dimitris Rizopoulos and Roula Tsonaka},
 title   = {The logistic transform for bounded outcome scores},
 journal = {Biostatistics},
 volume  = {8},
 number  = {1},
 pages   = {72-85},
 year    = {2007},
}

@Article{lia+zeg86,
 author  = {Kung-Yee Liang and Scott Zeger },
 title   = {Longitudinal data analysis using generalized linear models},
 journal = {Biometrika},
 volume  = {73},
 number  = {1},
 pages   = {1322},
 year    = {1986},
}

@Book{mad86,
 author  = {G. S. Maddala},
 title   = {Limited-dependent and qualitative variables in econometrics},
 edition = {},
 publisher={Cambridge University Press},
 address = {Cambridge},
 year    = {1986},
}

@Book{mcc+nel89,
 author  = {P. McCullagh and J. A. Nelder},
 title   = {Generalized linear models},
 edition = {Second},
 publisher={Chapman and Hall},
 address = {London},
 year    = {1989},
}

@Book{mcq+tsa98,
 author  = {A. McQuarrie and A. Tsai},
 title   = {Regression and times series model selection},
 edition = {},
 publisher={World Scientific Publishing Company},
 address = {New Jersey},
 year    = {1998},
}

@Book{mad83,
 author  = {G. S. Maddala},
 title   = {Limited-dependent and qualitative variables in econometric},
 edition = {Second},
 publisher={Cambridge University Press},
 address = {Cambridge},
 year    = {1983},
}

@book{mccullagh1989generalized,
  title={Generalized linear models},
  author={McCullagh, Peter and Nelder, John A},
  edition = {2},  
  year={1989},
  address = {London},  
  publisher={CRC press}
}

@Techreport{mit09,
 author  = {Pablo A. Mitnik},
 title   = {The Kumaraswamy distribution: a median-dispersion re-parametrization for regression modeling and simulation-based estimation},
institution = {Department of Sociology, University of Wisconsin-Madison},
year    = {2009},
Type = {Relatório técnico},
}

@mastersthesis{miy08,
Author = {Eliane Shizue Miyashiro},
Title = {Modelos de regressão beta e simplex para análise de proporções},
School = {Instituto de Matemática e Estatística - Universidade de São Paulo},
Year = {2008},
Type = {Dissertação de mestrado em estatística},
}

@inproceedings{mou+ist07,
 author  = {Claudia S. Moura and Márcia Istake},
 title   = {Principais determinantes do valor do rendimento das aposentadorias no Brasil e no Paraná para o ano de 2004},
 booktitle = {V Ecopar},
 year    = {2007},
}

@Article{mul86,
 author  = {J. Mullahi},
 title   = {Specification and testing of some modified count data models},
 journal = {Journal of Econometrics},
 volume  = {33},
 number  = {},
 pages   = {341-365},
 year    = {1986},
}

@Book{noc+wri06,
 author  = {J. Nocedal and S. J. Wright},
 title   = {Numerical Optimization},
 edition = {2},
 publisher={Springer},
 address = {New York},
 year    = {2006},
}

@phdthesis{osp08,
Author = {Raydonal Ospina},
Title = {Modelos de regressão beta inflacionados},
School = {Instituto de Matemática e Estatística - Universidade de São Paulo},
Year = {2008},
Type = {PhD thesis},
}

@Article{osp+cri+vas06,
 author  = {Raydonal Ospina and Francisco Cribari-Neto and Klaus L. P. Vasconcellos},
 title   = {Improved point and interval estimation for a beta regression model},
 journal = {Computational Statistics and Data Analysis},
 volume  = {51},
 number  = {2},
 pages   = {960-981},
 year    = {2006},
}

@Article{osp+fer08,
 author  = {Raydonal Ospina and Silvia Lopes Paula Ferrari},
 title   = {Inflated beta distributions},
 journal = {Statistical Papers},
 volume  = {51},
 number  = {1},
 pages   = {111-126},
 year    = {2010},
}

@Techreport{reg+art08,
author  = {Daniel Evangelista Régis and Rinaldo Artes},
title   = {Modelo Multi-Estado de Markov em Cartões de Crédito},
institution = {Insper},
year    = {2008},
Type = {Technical report},
}

@Article{osp+fer11,
 author  = {Raydonal Ospina and Silvia Lopes Paula Ferrari},
 title   = {A general class of zero-or-one inflated beta regression models},
 journal = {Computational Statistics and Data Analysis,},
 volume  = {in press},
 number  = {},
 pages   = {},
 year    = {2011},
}

@Book{pac+sal97,
 author  = {Luigi Pace and Alessandra Salvan},
 title   = {Principles of Statistical Inference from a Neo-Fisherian Perspective},
 edition = {},
 publisher={World Scientific},
 address = {Singapore},
 year    = {1997},
}

@Article{pao01,
 author  = {P. Paolino},
 title   = {Maximum likelihood estimation of models with beta-distributed dependent variables},
 journal = {Political Analysis},
 volume  = {9},
 number  = {4},
 pages   = {325-346},
 year    = {2001},
}

@Article{pap+woo96,
 author  = {L. Papke and J. Wooldridge},
 title   = {Econometric methods for fractional response variables with an application to 401(k) plan participation rates},
 journal = {Journal of Applied Econometrics},
 volume  = {11},
 number  = {},
 pages   = {619-632},
 year    = {1996},
}

@inproceedings{per+cri10,
 author  = {Tarciana Liberal Pereira and Francisco Cribari-Neto},
 title   = {A test for correct model specification in inflated beta regressions},
 booktitle = {Sinape 19},
 address = {São Pedro:Brasil},
 note = {},
 year = {2010},
}

@Article{per+bot+san11a,
 author  = {Gustavo Henrique Araujo Pereira and Denise Aparecida Botter and Mônica Carneiro Sandoval},
 title   = {The truncated inflated beta distribution},
 journal = {Communications in Statistics - Theory and Methods,},
 volume  = {in press},
 number  = {},
 pages   = {},
 year    = {2011},
}

@inproceedings{per+bot+san11b,
 author  = {Gustavo Henrique Araujo Pereira and Denise Aparecida Botter and Mônica Carneiro Sandoval},
 title   = {Modelos de regressão beta inflacionados truncados},
 booktitle = {Escola de Modelos de Regressão 12},
 address = {Fortaleza:Brasil},
 note = {},
 year = {2011},
}

@mastersthesis{pin09,
Author = {Eliane Cantinho Pinheiro},
Title = {Ajustes para o teste da razão de verossimilhanças em modelos de regressão beta},
School = {Instituto de Matemática e Estatística - Universidade de São Paulo},
Year = {2009},
Type = {Dissertação de mestrado em estatística},
}

@Article{pin+fer09,
 author  = {Silvia Lopes Paula Ferrari and Eliane Cantinho Pinheiro},
 title   = {Improved likelihood inference in beta regression},
 journal = {Journal of Statistical Computation and Simulation},
 volume  = {, in press},
 number  = {},
 pages   = {},
 year    = {2009},
}

@Article{poo+poo99,
 author  = {W. Y. Poon and Y. S. Poon},
 title   = {Conformal normal curvature and assessment of local influence},
 journal = {Journal of the Royal Statistical Society Series B},
 volume  = {61},
 number  = {},
 pages   = {51-61},
 year    = {1999},
}

@Article{ram+sil09,
 author  = {Joaquim J. S. Ramalho and Jacinto Vidigal Silva},
 title   = {A two-part fractional regression model for the financial leverage decisions of micro, small, medium and large firms},
 journal = {Quantitative finance},
 volume  = {9},
 number  = {5},
 pages   = {621-636},
 year    = {2009},
}

@inproceedings{rid+dem+hin98,
 author  = {M. Ridout and C. G. B. Demétrio and J. Hinde},
 title   = {Models for count data with many zeros},
 booktitle = {International Biometric Conference - IBC 98, Cape Town},
 address = {Cape Town, África do Sul},
 note = {179-192},
 year = {1998},
}

@Article{rig+sta05,
 author  = {R. A. Rigby and D. M. Stasinopoulos},
 title   = {Generalized additive models for location, scale and shape},
 journal = {Journal of the Royal Statistics Society: Series C (Applied Statistics)},
 volume  = {54},
 number  = {3},
 pages   = {507-554},
 year    = {2005},
}

@Article{rob07,
 Author = {Cliff A. Robb and Deanna L. Sharpe},
 Title = {Effect of personal financial knowledge on college students credit card behavior},
 journal = {Journal of Financial Counseling and Planning},
 volume  = {20},
 number  = {1},
 pages   = {25-43},
 Year = {2009},
}

@Article{roc+sim11,
 author  = {Alexandre B. Simas and Andréa V. Rocha},
 title   = {Influence diagnostics in a general class of beta regression models},
 journal = {Test},
 volume  = {20},
 number  = {},
 pages   = {95-119},
 year    = {2011},
}

@Article{seb+nya00,
 author  = {G. A. F. Seber and S. O. Nyangoma},
 title   = {Residuals for multinomial models},
 journal = {Biometrika},
 volume  = {87},
 number  = {1},
 pages   = {183-191},
 year    = {2000},
}

@Book{sen+sin+lim10,
 author  = {P. K. Sen and J. M. Singer and A. C. P. Lima},
 title   = {From Finite Sample to Asymptotic Methods in Statistics},
 edition = {},
 publisher={Cambridge University Press},
 address = {New York},
 year    = {2010},
}

@Article{sim+bar+roc10,
 author  = {Alexandre B. Simas and Wagner Barreto-Souza and Andréa V. Rocha},
 title   = {Improved estimators for a general class of beta regression models},
 journal = {Computational Statistics and Data Analysis},
 volume  = {54},
 number  = {},
 pages   = {348-366},
 year    = {2010},
}

@Article{smi+ver06,
 author  = {M. Smithson and J. Verkuilen},
 title   = {A better lemon squeezer? Maximum likelihood regression with beta-distributed
 dependent variables},
 journal = {Psychological Methods},
 volume  = {11},
 number  = {},
 pages   = {54-71},
 year    = {2006},
}

@Incollection{ste86,
 author  = {M. A. Stephens},
 title   = {Tests based on EDF statistics},
 booktitle = {Goodness-of-fit techniques},
 publisher={Marcel Dekker},
 address = {New York},
 year    = {1986},
 editor = {R B. D´Agostino and M. A. Stephens},
}

@Article{ter02,
 author  = {G. R. Terrell},
 title   = {The gradient statistics},
 journal = {Computing Science and Statistics},
 volume  = {34},
 number  = {},
 pages   = {206-215},
 year    = {2002},
}

@Book{tho+ede+cro02,
 author  = {L. C. Thomas and D. B. Edelman and J. N. Crook},
 title   = {Credit scoring and its applications},
 edition = {},
 publisher={Siam},
 address = {Philadelphia},
 year    = {2002},
}

@Techreport{tod+all02,
 author  = {E. Toder and L. Thompson and M. Fraveault and R. Johnson and K. Perese and C. Ratcliffe and K. Smith and C. Uccello and T. Waidmann and J. Berk and R. Woldemariam and G. Burtless and C. Sahm and D. Wolf},
 title   = {Modeling income in the near term: revised projections of retirement income through 2020 for the 1931-1960 birth cohorts},
institution = {The Urban Institute},
year    = {2002},
Type = {Relatório técnico},
}

@Article{tu02,
 author  = {W. Tu},
 title   = {Zero inflated data},
 journal = {Encyclopedia of Environmetrics},
 volume  = {4},
 number  = {},
 pages   = {2387-2391},
 year    = {2002},
}

@Article{vas+cri05,
 author  = {K. L. P. Vasconcellos and F. Cribari-Neto},
 title   = {Improved maximum likelihood estimation in a new class of beta regression models},
 journal = {Brazilian Journal of Probability and Statistics},
 volume  = {19},
 number  = {},
 pages   = {13-31},
 year    = {2005},
}

@phdthesis{ven08,
Author = {Maria Kelly Venezuela},
Title = {Equação de estimação generalizada e influência local para modelos de regressão beta com medidas repetidas},
School = {Instituto de Matemática e Estatística - Universidade de São Paulo},
Year = {2008},
Type = {Tese de doutorado em estatística},
}

@Book{ver+mol00,
 author  = {Geert Verbeke and Geert Molenberghs},
 title   = {Linear mixed models for longitudinal data},
 edition = {},
 publisher={Springer-Verlag},
 address = {New York},
 year    = {2000},
}

@Article{vie+hin+dem00,
 author  = {A. M. C. Vieira and J. P. Hinde and C. G. B. Demétrio},
 title   = {Zero inflated proportion data models applied to a biological control assay},
 journal = {Journal of Applied Statistics},
 volume  = {27},
 number  = {3},
 pages   = {373-389},
 year    = {2000},
}

@Article{wed74,
 author  = {R. W. M. Wedderburn},
 title   = {Quasi-likelihood function, generalized linear models, and the Gauss-Newton method},
 journal = {Biometrika},
 volume  = {61},
 number  = {3},
 pages   = {439-447},
 year    = {1974},
}


@Article{zim10,
 author  = {Daniel Zimprich},
 title   = {Modeling change in skewed variables using mixed beta regression models},
 journal = {Research in Human Development},
 volume  = {7},
 number  = {1},
 pages   = {9-26},
 year    = {2010},
}



